A General Framework For Detecting Anomalous Inputs to DNN Classifiers

Detecting anomalous inputs, such as adversarial and out-of-distribution (OOD) inputs, is critical for classifiers (including deep neural networks or DNNs) deployed in real-world applications. While prior works have proposed various methods to detect such anomalous samples using information from the internal layer representations of a DNN, there is a lack of consensus on a principled approach for the different components of such a detection method. As a result, often heuristic and one-off methods are applied for different aspects of this problem. We propose an unsupervised anomaly detection framework based on the internal DNN layer representations in the form of a meta-algorithm with configurable components. We proceed to propose specific instantiations for each component of the meta-algorithm based on ideas grounded in statistical testing and anomaly detection. We evaluate the proposed methods on well-known image classification datasets with strong adversarial attacks and OOD inputs, including an adaptive attack that uses the internal layer representations of the DNN (often not considered in prior work). Comparisons with five recently-proposed competing detection methods demonstrates the effectiveness of our method in detecting adversarial and OOD inputs.

==> Contents/related_works_bak.tex <==
%% DO NOT EDIT
\section{Related Works}
\label{sec:related}
We categorize and review some prior works on adversarial and OOD detection. A more detailed survey and taxonomy of anomaly detection methods in deep learning can be found in \cite{bulusu2020survey}.

\smallskip
\noindent{\bf Supervised Methods}

In \cite{lee2018simple}, the layer representations of a DNN are modeled class-conditionally using multivariate Gaussian densities, which leads to the Mahalanobis distance from the mean vector as a layer feature. The feature vector of Mahalanobis distances from the layers is used to train a binary logistic classifier for discriminating adversarial (or OOD samples) from natural samples. \cite{ma2018characterizing_iclr} propose using the LID of layer representations of a DNN as a feature for characterizing adversarial samples. Similar to the approach of \cite{lee2018simple}, they calculate a feature vector of LID estimates from the layer representations, which is used for training a logistic classifier for discriminating adversarial samples from natural samples. In \cite{yang2019ml}, feature attribution methods are used to characterize the input and intermediate layer representations of a DNN. They find that adversarial inputs drastically alter the feature attribution map compared to natural inputs. Measures such as the inter-quartile range and median absolute deviation are used to quantify the dispersion in the distribution of attribution values, which are then used as features to train a logistic classifier for discriminating adversarial samples from natural samples.

\smallskip
\noindent{\bf Unsupervised Methods}

\cite{roth2019odds} show that the log-odds ratio of inputs to a classifier (not necessarily a DNN) can reveal some interesting properties of adversarial inputs. They propose test statistics based on the expected log-odds of noise-perturbed inputs from different source and predicted class pairs, which are suitably normalized and thresholded to detect adversarial inputs. They also propose a reclassification method for correcting the classifier's prediction on adversarial inputs. This is based on training logistic classifiers (one for each predicted class) that use the expected noise-perturbed log-odds ratio as features. In \cite{zheng2018robust}, the class-conditional distributions of fully-connected intermediate layer representations are modeled using Gaussian mixture models~\footnote{Convolutional layers are not modeled in their approach.}. Inputs with a likelihood lower than a (class-specific) threshold under each class-conditional mixture model are rejected as adversarial. 
In \cite{miller2019ada}, an anomaly detection method focusing on adversarial attacks is proposed, which in its basic form can be described as follows.
The class-conditional density of the layer representations of a DNN are modeled using Gaussian mixture models, and they are used to calculate a Bayes class posterior at each layer. The Kullback-Leibler divergence between the class posterior of the DNN (based on the softmax function) and the estimated Bayes class posterior from each layer are used as test statistics for detecting adversarial samples. A number of variations of this test statistic that lead to improved detection are also proposed.
%
\cite{sastry2019gram} propose a method for detecting OOD samples based on analyzing the Gram matrices of the layer representations (activations) of a DNN. 
The Gram matrices of different orders (order $1$ corresponds to the standard definition) capture the pairwise correlations between the elements of a layer activation. 
At training time, their detector records the element-wise minimum and maximum values of the Gram matrices (of different orders) from a training set of natural inputs, conditioned on each predicted class. The extent of deviation from the minimum and maximum values observed at training time is used to calculate a class-specific deviation test statistic at each layer. The final score for OOD detection is obtained by adding up the normalized deviations from the layers, where the normalization factor for a layer is the expected deviation observed on a held-out validation dataset~\footnote{\textcolor{red}{(Move discussion to text)} We note that the deviation statistic based on Gram matrices from the layer activations defined by \cite{sastry2019gram} can be used as a test statistic for \proposed as well. Different from \cite{sastry2019gram}, \proposed would combine the layerwise, class-conditional p-values estimated from the test statistics into an adversarial score or OOD score (\S~\ref{sec:scoring_adver}).}.

\smallskip
\noindent{\bf Confidence Metrics for Classifiers}

Works such as the trust score~\cite{jiang2018trust} and deep KNN~\cite{papernot2018deep} have explored the problem of developing a confidence metric that can be used to independently validate the predictions of a classifier. Inputs with a low confidence score are expected to be mis-classified and can be flagged as potentially adversarial or OOD. 
The deep KNN method~\cite{papernot2018deep} uses the class labels of the k-nearest neighbors of DNN layer representations to calculate a non-conformity score corresponding to each class. Large values of non-conformity corresponding to the predicted class indicate that an input may not have a reliable prediction. The method calculates empirical p-values of the non-conformity scores to provide a confidence score, credibility score, and an alternate (corrected) class prediction for test inputs. 
The trust score~\cite{jiang2018trust} estimates the $\alpha$-high density (level) set for each class, and calculates the distances from a test point to the $\alpha$-high density sets from the classes to define a confidence metric. These methods can also be categorized as unsupervised.
%Cite 'jha2019abc' for confidence metrics in the camera ready version


==> algo_detailed.tex <==
% Detailed algorithm for the appendix
\begin{algorithm}[htb]
	\caption{Meta-algorithm for Anomaly Detection}
	\label{meta_algorithm_detailed}
	% Next two lines reduce the font size. Comment if needed
	\algsetup{linenosize=\small}
    \small
	\begin{algorithmic}
	    \STATE {\bfseries Inputs:} Trained DNN $\mathbf{F}(\cdot)$, Dataset $\mathcal{D}$, Test input $\bfx$, \\FPR $\alpha$ or detection threshold $\tau$.
		\STATE {\bfseries Output:} Detector decision -- normal $0$ or anomaly $1$.
		\medskip
		%\STATE {\bf Preprocessing:}
		%\begin{ALC@g}
		\STATE Calculate the detection threshold $\tau$ (if not specified).
		\STATE Class prediction of $\,\bfx$: $\hat{c} = \argmax_{c \in [m]} F_c(\bfx)$.
		\STATE Layer representations of $\,\bfx$: $\bfx^{(\ell)} = \mathbf{f}_\ell(\bfx), \,\forall \ell \in \mathcal{L}$.
		\STATE Data subsets: $\widehat{\mathcal{D}}_a(\ell, \hat{c})$ and $\mathcal{D}_a(\ell, c), \,\forall \,\ell \in \mathcal{L}, \,c \in [m]$.
		%\end{ALC@g}
		\smallskip
		\STATE {\bf I. Test statistics}:
		\begin{ALC@g}
		    %\STATE For each layer $\,\ell \in \mathcal{L}$:
		    \NoDo
		    \FOR{each layer $\,\ell \in \mathcal{L}$:}
		    %\begin{ALC@g}
		        \STATE Calculate $\,t^{(\ell)}_{p \cond \hat{c}} \,=\, T(\bfx^{(\ell)}, \hat{c}, \widehat{\mathcal{D}}_a(\ell, \hat{c}))$.
		        \STATE Calculate $\,t^{(\ell)}_{s \cond c} \,=\, T(\bfx^{(\ell)}, c, \mathcal{D}_a(\ell, c)), ~\forall c \in [m]$.
            %\end{ALC@g}
            \ENDFOR 
            \smallskip
            \STATE Compile the vectors: $\bft^{}_{p \cond \hat{c}}, \bft^{}_{s \cond 1}, \cdots, \bft^{}_{s \cond m}$.
        \end{ALC@g}
        \smallskip
        \STATE {\bf II. Normalizing transformations}:
        \begin{ALC@g}
            \NoThen
            \IF{multivariate normalization:}
                %\STATE Normalize the $\,m + 1\,$ test statistic vectors.
                \STATE Calculate $\,q(\bft_{p \cond \hat{c}}), q(\bft_{s \cond 1}), \cdots, q(\bft_{s \cond m})$.
            \ELSE
                \NoDo
                \FOR{each layer $\,\ell \in \mathcal{L}$:}
                    \STATE Calculate $\,q(t^{(\ell)}_{p \cond \hat{c}}), q(t^{(\ell)}_{s \cond 1}), \cdots, q(t^{(\ell)}_{s \cond m})$.
                \ENDFOR
                \smallskip
                %\STATE {\bf [Optional]}
                \OptDo
                \FOR{each layer pair $\,(\ell_1, \ell_2) \in \mathcal{L}^2$:}
                    \STATE Calculate $\,q(t^{(\ell_1)}_{p \cond \hat{c}}, t^{(\ell_2)}_{p \cond \hat{c}})$.
                    \STATE Calculate $\,q(t^{(\ell_1)}_{s \cond 1}, t^{(\ell_2)}_{s \cond 1}), \cdots, q(t^{(\ell_1)}_{s \cond m}, t^{(\ell_2)}_{s \cond m})$.
                \ENDFOR
            \ENDIF
        \end{ALC@g}
        \smallskip
        \STATE {\bf III. Layerwise aggregation and scoring}:
        \begin{ALC@g}
            \NoThen
            \IF{multivariate normalization:}
                \STATE Set $\,q^{}_{\textrm{agg}}(\bft_{p \cond \hat{c}}) \,=\, q(\bft_{p \cond \hat{c}})$.
                \STATE Set $\,q^{}_{\textrm{agg}}(\bft_{s \cond c}) \,=\, q(\bft_{s \cond c}), ~\forall c \in [m]$.
            \ELSE
                \STATE Create the sets $\,Q_{p \cond \hat{c}}\,$ and $\,Q_{s \cond c}, ~\forall c \in [m]$.
                \STATE Calculate $\,q^{}_{\textrm{agg}}(\bft_{p \cond \hat{c}}) \,=\, r(Q_{p \cond \hat{c}})\,$.
                \STATE Calculate $\,q^{}_{\textrm{agg}}(\bft_{s \cond c}) \,=\, r(Q_{s \cond c}), ~\forall c \in [m]$.
            \ENDIF
            \smallskip
            \STATE Calculate the final score:\\$S(q^{}_{\textrm{agg}}(\bft_{p \cond \hat{c}}), q^{}_{\textrm{agg}}(\bft_{s \cond 1}), \cdots, q^{}_{\textrm{agg}}(\bft_{s \cond m}), \hat{c})\,$.
        \end{ALC@g}
        \smallskip
        \STATE {\bf IV. Detection decision}:
        \begin{ALC@g}
            \NoThen
            \IF{$S(q^{}_{\textrm{agg}}(\bft_{p \cond \hat{c}}), q^{}_{\textrm{agg}}(\bft_{s \cond 1}), \cdots, q^{}_{\textrm{agg}}(\bft_{s \cond m}), \hat{c}) \,\geq\, \tau$:}
                \STATE Return anomaly ($1$).
            \ELSE
                \STATE Return normal ($0$).
            \ENDIF
            %\STATE Return $\,\psi^{}_{\tau}(\bfx^{(0)}, \cdots, \bfx^{(L)}, \hat{c})$.
        \end{ALC@g}
	\end{algorithmic}
\end{algorithm}
%


==> scratch.tex <==

%Wrapfig version. Does not look good
\begin{wrapfigure}{L}{0.5\textwidth}
\vspace{-10mm}
\centering
\includegraphics[width=0.48\textwidth]{Figures/adversarial-detection-overview.pdf}
%\includegraphics[scale=0.3]{Figures/adversarial-detection-overview.pdf}
\caption{Overview of the proposed detection framework.}
\vspace{-10mm}
\label{fig:overview}
\end{wrapfigure}

\begin{figure*}[htb]
%\vspace{-3mm}
  \centering
  %\includegraphics[width=0.75\textwidth]{Figures/adversarial-detection-overview.pdf}
  %\includegraphics[scale=0.45]{Figures/adversarial-detection-overview.pdf}
  \includegraphics[height=0.35\textheight]{Figures/adversarial-detection-overview.pdf}
  \caption{Overview of the proposed detection framework. The DNN classifies a test input $\mathbf{x}$ into one of the $m$ classes. \proposed uses the predicted class and the layer representations to calculated class-conditional test statistics at each layer. The class-conditional test statistics from the layers are combined into class-conditional p-value estimates, which are then used by the decision function to determine whether the input is natural or anomalous. \proposed also provides a corrected prediction for the true class of the input, which is useful when the input is detected as adversarial.}
\vspace{-2mm}
\label{fig:overview}
\end{figure*}


One such approach is to use the p-value, that calculates the probability of a test statistic taking values (as or) more extreme than the observed value~\cite{wasserman2013all}.
More generally, a p-value is defined as any transformation of the test statistic (possibly a vector), following the null hypothesis distribution, into a uniformly distributed probability~\cite{root2016learning}.
This provides a simple approach to normalize the class-conditional test statistics in the univariate and multivariate cases, as discussed next.


We propose to use p-values, that are widely applied in hypothesis testing to evaluate how extreme an observed test statistic is with respect to the null-hypothesis distribution, with smaller p-values corresponding to stronger evidence for rejecting the null hypothesis~\cite{wasserman2013all}.
Conventionally, a p-value is defined as the probability of a test statistic taking values (as or) more extreme than an observed value. More generally, it is defined as any transformation of the test statistic (possibly a vector), following the null-hypothesis distribution, into a uniformly-distributed probability~\cite{root2016learning}.
This provides a simple approach to normalize the class-conditional test statistics in the univariate and multivariate cases, as discussed next.












\section{Related Works}
\label{sec:related}
We categorize and review some prior works on adversarial and OOD detection. A more detailed survey and taxonomy of anomaly detection methods in deep learning can be found in \cite{bulusu2020survey}.

\smallskip
\noindent{\bf Supervised Methods}

\smallskip
\noindent{\bf Unsupervised Methods}

\smallskip
\noindent{\bf Confidence Metrics for Classifiers}


We categorize and review some closely-related prior works on adversarial and OOD detection. For works that are based on multiple layer representations of a DNN, we discuss how the methods fit into the proposed meta-algorithm for anomaly detection.

In \cite{lee2018simple}, the layer representations of a DNN are modeled class-conditionally using multivariate Gaussian densities, which leads to the Mahalanobis distance confidence score being used as a test statistic (feature) at the layers. The feature vector of Mahalanobis distances from the layers is used to train a binary logistic classifier for discriminating adversarial (or OOD samples) from natural samples. While this method uses the class-conditional densities of the layer representations, it uses a rather simple parametric model based on multivariate Gaussians, which may not be suitable for the intermediate layer representations (issues include high dimensionality, non-negative activations, and multimodality). Also, this method does not use the predicted class of the DNN; instead it finds the ``closest'' class corresponding to each layer representation. In the context of the meta-algorithm, this method does not explicitly apply a normalizing transformation to the test statistics. However, the Mahalanobis distance can be interpreted as the negative-log-density, which follows the Chi-squared distribution (at each layer) under the Gaussian density assumption. Finally, we note that using a binary logistic classifier is equivalent to using a weighted linear combination of the test statistics for scoring as shown in Appendix \ref{}.

\cite{ma2018characterizing_iclr} propose using the local intrinsic dimensionality (LID) of the layer representations as a test statistic for characterizing adversarial samples. Similar to the approach of \cite{lee2018simple}, they calculate a test statistic vector of LID estimates from the layer representations, which is used for training a logistic classifier for discriminating adversarial samples from natural samples. In the context of the meta-algorithm, this method does not calculate class-conditional test statistics. The LID is estimated based on the marginal distribution of the layer representation manifold. The LID test statistics are not normalized in any way, and using the logistic classifier implies that this method uses a weighted linear combination of the test statistics for scoring.

In \cite{yang2019ml}, feature attribution methods are used to characterize the input and intermediate layer representations of a DNN. They find that adversarial inputs drastically alter the feature attribution map compared to natural inputs. Statistical dispersion measures such as the inter-quartile range (IQR) and median absolute deviation (MAD) are used to quantify the dispersion in the distribution of attribution values, which are then used as test statistics (features) to train a logistic classifier for discriminating adversarial samples from natural samples. In the context of the meta-algorithm, this method does not calculate class-conditional test statistics. The test statistics based on IQR or MAD are not normalized in any way. Similar to \cite{lee2018simple} and \cite{ma2018characterizing_iclr}, this method uses a weighted linear combination of the test statistics for scoring.



supervised
feinman2017detecting
lee2018simple
ma2018characterizing_iclr
yang2019ml

unsupervised
zheng2018robust
li2017adversarial
miller2019ada
papernot2018deep
roth2019odds
sastry2019gram
xu2017feature1
jiang2018trust

